Formalizing Multimedia Recommendation through Multimodal Deep Learning

Recommender systems (RSs) offer personalized navigation experiences on online platforms, but recommendation remains a challenging task, particularly in specific scenarios and domains. Multimodality can help tap into richer information sources and construct more refined user/item profiles for recommendations. However, existing literature lacks a shared and universal schema for modeling and solving the recommendation problem through the lens of multimodality. This work aims to formalize a general multimodal schema for multimedia recommendation. It provides a comprehensive literature review of multimodal approaches for multimedia recommendation from the last eight years, outlines the theoretical foundations of a multimodal pipeline, and demonstrates its rationale by applying it to selected state-of-the-art approaches. The work also conducts a benchmarking analysis of recent algorithms for multimedia recommendation within Elliot, a rigorous framework for evaluating recommender systems. The main aim is to provide guidelines for designing and implementing the next generation of multimodal approaches in multimedia recommendation.

==> revisioni.tex <==
R1:  The empirical evaluation could be strengthened with more tuning details and reproducible scripts. Sharing more artifacts like data preprocessing code would improve reproducibility.

Inseriamo una tabella con gli hyper params esplorati! [FATTO]

==============================
R2: Novelty and potential for innovation details: a. The paper appears to apply concepts from the multimodal deep learning survey[1] to multimodal recommender systems, presenting a taxonomy that is relatively simple and straightforward. However, the adaptation does not seem to be specifically tailored to the particularities of recommender systems. For example, exploring how users interact with various modalities of items might provide valuable insights, rather than collectively addressing user/item/interaction to formulate the pipeline.

Specificare meglio come questo framework si applichi allo scenario di raccomandazione (!!!)

R2: b. While the mathematical formulation provided is straightforward, using a single mathematical notation, for instance, γ(∙), to denote a function that performs the early fusion of multimodal representations, it would be beneficial for the authors to elucidate how γ(∙)  is implemented across different works to enhance the comprehensibility of the methodology.

spiegare come γ(∙) viene usato nelle different implementazioni

R2: c. The discussion in Section 3.5 could benefit from a more in-depth exploration of how current works handle inference and define losses within the context of multimodal recommender systems.

vedi punto 1 del R2

R2: c. While the datasets employed in the study are relevant, their relatively small size may limit the generalizability of the findings. Incorporating at least one larger dataset could enhance the robustness and applicability of the results.

spiegare che i dataset usati sono i più comuni (come in recsys), l'aggiunta degli hyperparams puo' giustificare i parametri esplorati, non abbiamo risorse per fare dataset più corposi

R2: In Section 4, four instances of instantiating the proposed multimodal pipeline are presented. It may be beneficial to integrate this section with the respective methodology sections, allowing for the provision of additional examples from current works, thereby enriching the practical context and application discussions. Consider integrating Section 4 with the respective methodology sections for enriched practical context and combining the discussions on technical challenges and future directions for a cohesive narrative.

provare a fondere 3 e 4

======================================

R3: 1. Given the diversity of multimedia recommendation scenarios, doubts arise about the feasibility of a single theoretical and applicative formalization to encompass all cases.

va capito come fare (!!!)

R3: 2. This paper references many cases of multimedia recommendation, while the datasets are limited and cannot cover these cases. This raises concerns regarding the proposed method's adaptability to different tasks.

i dataset sono quelli più comuni per la parte recsys. Altri dataset che siano adatti agli altri scenari non sono pubblici

R3: 3. The choice between early or late multimodal fusion for practical application and its impact on performance improvement lacks an explicit decision-making logic.

vedi punto 1 di R2

R3: 4. The proposed method's framework may be considered oversimplified in comparison to its claimed generalization capabilities.

cosa intende?

R3: 5. To enhance the paper's empirical support, it is advisable to include quantified performance improvement measures.

2/3 baseline no multimodal su questi dataset [FATTO]

==> tables/evaluation.tex <==
\begin{table}[!t]
\caption{Four literature examples of multimodal frameworks for multimedia recommendation. For each work, we report the performed task, the considered modalities for each input to the system (e.g., user and item), the feature extraction and multimodal representation strategies, the multimodal fusion, and the adopted inference/loss functions.}
\label{tab:validation}
\setlength\tabcolsep{3pt}
\scriptsize
\renewcommand\tabularxcolumn[1]{m{#1}}
\centering
\begin{tabularx}{\textwidth}{llllllMMM}
\toprule
\textbf{Paper} & \textbf{Task} & \textbf{Input} & \textbf{Modalities} & \makecell[l]{\textbf{Multimodal}\\\textbf{Input Data}} & \makecell[l]{\textbf{Feature}\\\textbf{Extraction}} & \textbf{Multimodal Representation} & \textbf{Multimodal Fusion} & \textbf{Inference and Loss} \\ \cmidrule{1-9}
\multirow{6}{*}{\citet{DBLP:conf/mm/WeiWN0HC19}} & \multirow{3}{*}{\makecell[l]{Micro-video\\ recommendation}} & \multirow{3}{*}{User} & Visual & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \multirow{6}{*}{\parbox{\linewidth}{Coordinate, aggregation of node's neighborhood and  combination with the ego node. Projection in both aggregation and combination.}} & \multirow{6}{*}{\parbox{\linewidth}{Early, modalities are combined through element-wise addition.}} & \multirow{6}{*}{\parbox{\linewidth}{Inference via inner-product between final user and item embeddings. BPR is the optimization function.}}  \\ \cmidrule{4-4}
& & & Textual & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & & \\ \cmidrule{4-4}
& & & Audio & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & & \\ \cmidrule{3-6}
& & \multirow{3}{*}{Item} & Visual & Video frames & ResNet50 & & & \\ \cmidrule{4-6}
& & & Textual & \makecell[l]{Captions and\\ descriptions} & Sentence2Vector & & & \\ \cmidrule{4-6}
& & & Audio & Audio track & VGGish & & & \\ \cmidrule{1-9}
\multirow{3}{*}{\citet{DBLP:journals/tomccap/WangDJJSN21}} & \multirow{3}{*}{\makecell[l]{Food\\recommendation}} & User & Textual & Users' tweets & Bi-RNN \& CNN & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & Score prediction with MLP for user tags. Loss is cross-entropy. User embedding is later adopted for recommendation.\\ \cmidrule{3-6} \cmidrule{9-9}
& & \multirow{2}{*}{Item} & Visual & Video Frames & VGGNet-19 & \multirow{2}{*}{\parbox{\linewidth}{Coordinate, no particular operation performed.}} & \multirow{2}{*}{\parbox{\linewidth}{Early, modalities are combined through concatenation.}} & \multirow{2}{*}{\parbox{\linewidth}{User-item score prediction with MLP and cross-entropy.}}\\ \cmidrule{4-6} &  &  & Textual & Recipe ingredients & TextCNN & & & \\ \cmidrule{1-9}
\multirow{2}{*}{\citet{DBLP:conf/mm/HanWJD17}} & \multirow{2}{*}{\makecell[l]{Outfit fashion\\ compatibility}} & \multirow{2}{*}{Item} & Visual & Product images & InceptionV3 & \multirow{2}{*}{\parbox{\linewidth}{Joint, features are projected into a shared embedding space.}} & \cellcolor[HTML]{EFEFEF} & \parbox{\linewidth}{Visual modality used for the inference.} \\ \cmidrule{4-6} \cmidrule{9-9}
& & & Textual & Descriptions & One-hot-encode & & \cellcolor[HTML]{EFEFEF} & \parbox{\linewidth}{Textual modality used for the contrastive component of the loss function.} \\ \cmidrule{1-9}
\multirow{2}{*}{\citet{DBLP:conf/recsys/OramasNSS17}} & \multirow{2}{*}{\makecell[l]{Artist and song\\ recommendation}} & \multirow{2}{*}{Item} & Textual & Artist biography & Custom CNN & \multirow{2}{*}{\parbox{\linewidth}{Coordinate, textual and audio features normalized and optionally fed into two separate MLPs.}} & \parbox{\linewidth}{Early, either normalized features are concatenated and fed into a one-layer MLP, or multimodal representations are connected to the one-layer MLP.} & \parbox{\linewidth}{Inference via inner-product between user and final item embeddings. Cosine distance is the loss function.} \\ \cmidrule{4-6}
& & & Audio & \makecell[l]{Audio\\spectrogram} & Custom CNN & & & \\ \bottomrule
\end{tabularx}
\end{table}
